Tearing the Veil: interaction of the Orion Nebula with its neutral environment

We present HI 21cm observations of the Orion Nebula, obtained with the Karl G. Jansky Very Large Array, at an angular resolution of 7.2"x5.7" and a velocity resolution of 0.77 km/s. Our data reveal HI absorption towards the radio continuum of the HII region, and HI emission arising from the Orion Bar photon-dominated region (PDR) and from the Orion-KL outflow. In the Orion Bar PDR, the HI signal peaks in the same layer as the H2 near-infrared vibrational line emission, in agreement with models of the photodissociation of H2. The gas temperature in this region is approximately 540K, and the HI abundance in the interclump gas in the PDR is 5-10% of the available hydrogen nuclei. Most of the gas in this region therefore remains molecular. Mechanical feedback on the Veil manifests itself through the interaction of ionized flow systems in the Orion Nebula, in particular the Herbig-Haro object HH202, with the Veil. These interactions give rise to prominent blueward velocity shifts of the gas in the Veil. The unambiguous evidence for interaction of this flow system with the Veil shows that the distance between the Veil and the Trapezium stars needs to be revised downwards to about 0.4pc. The depth of the ionized cavity is about 0.7pc, which is much smaller than the depth and the lateral extent of the Veil. Our results reaffirm the blister model for the M42 HII region, while also revealing its relation to the neutral environment on a larger scale.

==> acknow.tex <==
\def\beginacknowledgements{             % to begin acknowledgements section
 \noindent{\it Acknowledgements.$\,$}
 \message{Acknowledgements}}

\def\endacknowledgements{               % to end acknowledgements section
 \endsection}

\def\acknowledgeDRAO{The Dominion Radio Astrophysical Observatory of the
 Herzberg Institute of Astrophysics is operated as a national facility by the
 National Research Council of Canada.\ }

\def\acknowledgeWSRT{The Westerbork Synthesis Radio Telescope is operated by
the Netherlands Foundation for Radio Astronomy (SRZM) which is financially
supported by the Netherlands Organization for Scientific Research (NWO).\ }

\def\acknowledgeKOSMA{The KOSMA $3\,\m$ radio telescope at Gornergrat-S\"ud
 Observatory is operated by the University of Cologne and supported by the
 Deutsche Forschungsgemeinschaft (DFG) through grant SFB--301, as well as
 special funding from the Land Nordrhein-Westfalen. The observatory is
 administered
 by the Hochalpine Forschungsstationen Jungfraujoch und Gornergrat, Bern.\ }

\def\acknowledgeIRAMPdBI{This work is based on observations carried out with the
 IRAM Plateau de Bure Interferometer. IRAM is supported by INSU/CNRS (France),
 MPG (Germany) and IGN (Spain).\ }

\def\acknowledgeIRAS{The Infra Red Astronomical Satellite (IRAS) was developed
 and operated by the Netherlands Agency for Aerospace Programs (NIVR), the
 U.S.\s
 National Aeronautics and Space Administration (NASA) and the U.K.\s Science
 and Engineering Research Council (SERC).\ }

\def\acknowledgeNRAO{The National Radio Astronomy Observatory is a facility of
the National Science Foundation operated under cooperative agreement by
Associated Universities, Inc.\ }

\def\acknowledgeASTRON{Van der Werf is supported by the Netherlands
 Foundation for Astronomical Research (ASTRON), with financial support of the
 Netherlands Organization for Scientific Research (NWO).\ }

\def\acknowledgeASTRONpart{Van der Werf was partly supported by the
 Netherlands Foundation for Astronomical Research (ASTRON), with financial
 support of the Netherlands Organization for Scientific Research (NWO).\ }

\def\acknowledgeWHT{The William Herschel Telescope is operated on the island
of La Palma by the Royal Greenwich Observatory in the Spanish Observatorio del
Roque de los Muchachos of the Instituto de Astrofisica de Canarias.\ }

\endinput


==> hyphens.tex <==
\hyphenation{ASTRON}                    % how to (not) break these words
\hyphenation{cloud-let cloud-lets}
\hyphenation{HVABG}
\hyphenation{MNRAS}
\hyphenation{Peim-bert}
\hyphenation{Schloerb}
\endinput


==> journals.tex <==
\def\rmxaa{Rev. Mex. Astron. Astr.}

\endinput


==> molec.tex <==
%--------------- molecules and molecular ions --------------------------------
%

\def\mbox{\hbox}           % for compatibility of TeX and LaTeX use 

\def\CHp{\ifmmode \mbox{\rm CH}^+           %   +
         \else {\rm CH}$^+$                 % CH
         \fi}

\def\CO#1{\ifnum#1=0                    % CO isotopes
           \ifmmode \mbox{\rm CO}
           \else {\rm CO}
           \fi
          \else
           \ifnum#1<15
            \ifmmode ^{#1}\mbox{\rm CO}
            \else $^{#1}${\rm CO}
            \fi
           \else
            \ifmmode \mbox{\rm C}^{#1}\mbox{\rm O}
            \else {\rm C}$^{#1}${\rm O}
            \fi
           \fi
          \fi}

\def\COp{\ifmmode \mbox{\rm CO}^+           %   +
         \else {\rm CO}$^+$                 % CO
         \fi}

\def\CS#1{\ifnum#1=0                    % CS isotopes
           \ifmmode \mbox{\rm CS}
           \else {\rm CS}
           \fi
          \else
           \ifnum#1<15
            \ifmmode ^{#1}\mbox{\rm CS}
            \else $^{#1}${\rm CS}
            \fi
           \else
            \ifmmode \mbox{\rm C}^{#1}\mbox{\rm S}
            \else {\rm C}$^{#1}${\rm S}
            \fi
           \fi
          \fi}

\def\HCOp{\ifmmode \mbox{\rm HCO}^+          %    +
          \else {\rm HCO}$^+$                % HCO
          \fi}

\def\HCtN{\ifmmode \mbox{\rm HC}_3\mbox{\rm N}     % HC N
          \else {\rm HC}$_3${\rm N}                %   3
          \fi}

\def\Hp{\ifmmode \mbox{\rm H}^+           %  +
        \else {\rm H}$^+$                 % H
        \fi}
                                                  %    +
\def\HtOp{\ifmmode \mbox{\rm H}_2\mbox{\rm O}^+   % H O
          \else {\rm H}$_2${\rm O}$^+$            %  2
          \fi}
                                                   %    +
\def\HthOp{\ifmmode \mbox{\rm H}_3\mbox{\rm O}^+   % H O
              \else {\rm H}$_3${\rm O}$^+$         %  3
              \fi}
                                            %  +
\def\Hthp{\ifmmode \mbox{\rm H}_3^+         % H
             \else {\rm H}$_3^+$            %  3
             \fi}

\def\Ht{\ifmmode \mbox{\rm H}_2              % H
        \else {\rm H}$_2$                    %  2
        \fi}

\def\HtCO{\ifmmode \mbox{\rm H}_2\mbox{\rm CO} % H CO
          \else {\rm H}$_2${\rm CO}            %  2
          \fi}

\def\HtO{\ifmmode \mbox{\rm H}_2\mbox{\rm O} % H O
         \else {\rm H}$_2${\rm O}            %  2
         \fi}
                                                   %  18
\def\HteO{\ifmmode \mbox{\rm H}_2^{18}\mbox{\rm O} % H O
          \else {\rm H}$_2^{18}${\rm O}            %  2
          \fi}

\def\OHp{\ifmmode \mbox{\rm OH}^+   %   +
         \else {\rm OH}$^+$         % OH
         \fi}
                                               %  +
%
%---------------------- atoms and atomic ions ---------------------------------
%

\def\ion#1#2{\ifmmode \mbox{{\rm #1}}\,\mbox{{\sc #2}} % generic ion
        \else {\rm #1}$\,${\sc #2}
        \fi}
\def\CI{\ion{C}{i}}
\def\CII{\ion{C}{ii}}
\def\FeII{\ion{Fe}{ii}}
\def\HI{\ion{H}{i}}
\def\HII{\ion{H}{ii}}
\def\NII{\ion{N}{ii}}
\def\NeII{\ion{Ne}{ii}}
\def\OI{\ion{O}{i}}
\def\OII{\ion{O}{ii}}
\def\OIII{\ion{O}{iii}}
\def\SII{\ion{S}{ii}}
\def\SIII{\ion{S}{iii}}
\def\SiII{\ion{Si}{ii}}
\def\SiVI{\ion{Si}{vi}}

%
%-------------------- hydrogen recombination lines ---------------------------
%

\def\rec#1#2{\if#2a                            % generic
              \ifmmode \mbox{{\rm #1}}\alpha   % recombination line
              \else {\rm #1}$\alpha$
              \fi
             \fi
             \if#2b
              \ifmmode \mbox{{\rm #1}}\beta
              \else {\rm #1}$\beta$
              \fi
             \fi
             \if#2g
              \ifmmode \mbox{{\rm #1}}\gamma
              \else {\rm #1}$\gamma$
              \fi
             \fi}

\def\Lya{\rec{Ly}{a}}                          % Lyman alpha
\def\Ha{\rec{H}{a}}                            % H alpha
\def\Hb{\rec{H}{b}}                            % H beta
\def\Paa{\rec{Pa}{a}}                          % Paschen alpha
\def\Pab{\rec{Pa}{b}}                          % Paschen beta
\def\Bra{\rec{Br}{a}}                          % Brackett alpha
\def\Brg{\rec{Br}{g}}                          % Brackett gamma

\endinput


==> refs.tex <==
%..............................................................................
%
%             This is    r e f s . t e x
%
% A LaTeX file for keeping tracks of references to figures, sections,
% tables and equations.
%
% Latest update: Paul van der Werf 06-Jan-2000
%
%..............................................................................

\newcommand{\tabref}[1]{Table~\protect\ref{#1}}
\newcommand{\figref}[1]{Fig.~\protect\ref{#1}}
\newcommand{\figrefbare}[1]{\protect\ref{#1}}
\newcommand{\figrefs}[1]{Figs.~\protect\ref{#1}}
\newcommand{\figsref}[2]{Figs.~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\twofigsref}[2]{Figs.~\protect\ref{#1} and~\protect\ref{#2}}
\newcommand{\eqref}[1]{Eq.~$\left(\protect\ref{#1}\right)$}
\newcommand{\eqsref}[2]{Eqs.~$\left(\protect\ref{#1}\right)$--$\left(\protect\ref{#2}\right)$}
\newcommand{\twoeqsref}[2]{Eqs.~$\left(\protect\ref{#1}\right)$--$\left(\protect\ref{#2}\right)$}
\newcommand{\secref}[1]{Sect.~\protect\ref{#1}}
\newcommand{\secsref}[2]{Sects.~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\twosecsref}[2]{Sects.~\protect\ref{#1} and~\protect\ref{#2}}

% upper case versions to begin sentences: 

\newcommand{\Tabref}[1]{\tabref{#1}}
\newcommand{\Figref}[1]{Figure~\protect\ref{#1}}
\newcommand{\Figrefs}[1]{Figures~\protect\refs{#1}}
\newcommand{\Figsref}[2]{Figures~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\Eqref}[1]{Equation~(\protect\ref{#1})}
\newcommand{\Eqsref}[2]{Equations~(\protect\ref{#1})--(\protect\ref{#2})}
\newcommand{\Secref}[1]{Section~\protect\ref{#1}}

\endinput


==> symbols.tex <==
\def\mbox{\hbox}           % for compatibility of TeX and LaTeX use

%------------------ degrees, magnitudes, RA, Dec etc -------------------------
%

\def\deg{\ifmmode ^\circ                % degrees symbol
         \else $^\circ$
         \fi
         \hskip -0.1truecm}
\def\degd#1.#2{                         % degrees over decimal point
                                        % syntax: \degd 4.3 or \degd 4.{34}
               \ifmmode {#1^{\hskip 0.05em\circ}\hskip-0.42em.\hskip0.08em#2}
               \else {#1$^{\hskip 0.05em\circ}\hskip-0.42em.\hskip0.08em$#2}
               \fi
              }
\def\mind#1.#2{                         % minutes over decimal point
                                        % syntax: \mind 4.3
               \ifmmode {#1^{\hskip 0.05em\prime}\hskip-0.35em.\hskip0.05em#2}
               \else {#1$^{\hskip 0.05em\prime}\hskip-0.35em.\hskip0.05em$#2}
               \fi
              }
\def\secd#1.#2{                         % seconds over decimal point
                                        % syntax: \secd 4.3
               \ifmmode {#1^{\prime\prime}\hskip-0.46em.\hskip0.12em#2}
               \else {#1$^{\prime\prime}\hskip-0.46em.\hskip0.12em$#2}
               \fi
              }
\def\timsecd#1.#2{                      % time seconds over decimal point
                                        % syntax: \timsecd 4.3
                  \ifmmode {#1^{\rm s}\hskip-0.39em.\hskip0.08em#2}
                  \else {$#1^{\rm s}\hskip-0.39em.\hskip0.08em#2$}
                  \fi
                 }
\def\hms#1h#2m#3s{                      % hms format (for RA)
                                        % syntax: \hms 12h34m45s
                  \relax
                  \ifmmode #1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                  \else \hbox{$#1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}$}
                  \fi
                 }
\def\dms#1d#2m#3s{                      % dms format (for Dec)
                                        % syntax: \dms 12d14m45s
                  \relax
                  \ifmmode #1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                  \else \hbox{$#1^\circ\,#2^{\prime}\,#3^{\prime\prime}$}
                  \fi
                 }
\def\dmsd#1d#2m#3.#4s{                  % dms format with decimal point (Dec)
                                        % syntax: \dmsd 12d13m34.5s
                      \relax
                      \ifmmode #1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                               \hskip-0.46em.\hskip0.12em#4
                      \else \hbox{$#1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                            \hskip-0.46em.\hskip0.12em#4$}
                      \fi
                     }
\def\hm#1h#2m{                          % hm format (for RA)
                                        % syntax: \hm 12h13m
              \relax
              \ifmmode #1^{\rm h}\,#2^{\rm m}
              \else \hbox{$#1^{\rm h}\,#2^{\rm m}$}
              \fi
             }
\def\dm#1d#2m{                          % dm format (for Dec)
                                        % syntax: \dm 12d13m
              \relax
              \ifmmode #1^\circ\,#2^{\prime}
              \else \hbox{$#1^\circ\,#2^{\prime}$}
              \fi
             }
\def\hmsd#1h#2m#3.#4s{                  % hms format with decimal point (RA)
                                        % syntax: \hmsd 12h13m34.5s
                      \relax
                      \ifmmode #1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                               \hskip-0.39em.\hskip0.08em#4
                      \else \hbox{$#1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                            \hskip-0.39em.\hskip0.08em#4$}
                      \fi
                     }
\def\hmd#1h#2.#3m{                  % hm format with decimal point (RA)
                                    % syntax: \hmd 12h13.6m
                  \relax
                  \ifmmode #1^{\rm h}\,#2^{\rm m}
                           \hskip-0.55em.\hskip0.22em#3
                  \else \hbox{$#1^{\rm h}\,#2^{\rm m}
                        \hskip-0.55em.\hskip0.22em#3$}
                  \fi
                 }
\def\mg{\relax                          % magnitudes symbol
        \ifmmode ^{\rm m}
        \else $^{\rm m}$
        \fi
       }
\def\mgd#1.#2{                          % magnitudes over decimal point
                                        % syntax: \mgd 4.3
              \relax
              \ifmmode #1^{\rm m}
                       \hskip-0.55em.\hskip0.22em#2
              \else \hbox{#1$^{\rm m}
                    \hskip-0.55em.\hskip0.22em$#2}
              \fi
             }

%
%-------------------- math symbols --------------------------------------------
%

\def\la{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\ga{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}

%
%--------------------------- units -------------------------------------------
% use: e.g. $15\kms$
%

\def\unitspace{\;}                      % space to be used with units

\def\un#1{\ifmmode \unitspace\mbox{\rm #1} % generic unit
          \else $\unitspace$#1
          \fi}
\def\pun#1#2{\ifmmode \unitspace\mbox{\rm #1}^{#2} % generic unit with a power
             \else $\unitspace$#1$^{#2}$
             \fi}
\def\per#1{\ifmmode \unitspace\mbox{\rm #1}^{-1} % generic unit with power -1
           \else $\unitspace$#1$^{-1}$
           \fi}

\def\Ang{\un{\AA}}                    % Angstrom
\def\AU{\un{AU}}                      % AU
\def\cm{\un{cm}}                      % cm
\def\es{\un{erg}\ps}                  %      -1
                                      % erg s
\def\esc{\es\pcmsqu}                  %      -1 -2
                                      % erg s cm
\def\escmum{\esc\mum^{-1}}            %      -1 -2  -1
                                      % erg s cm  mu
\def\escs{\esc\pun{sr}{-1}}           %      -1 -2 -1
                                      % erg s cm sr
\def\escsm{\escs\mum^{-1}}            %      -1 -2 -1 -1
                                      % erg s cm sr mu
\def\Eu{\font\euro = eurorm {\euro E}} % Euro
\def\eV{\un{eV}}                      % eV
\def\GHz{\un{GHz}}                    % GHz
\def\Jy{\un{Jy}}                      % Jy
\def\K{\un{K}}                        % K
\def\kms{\un{km}\pun{s}{-1}}          %     -1
                                      % km s
\def\kpc{\un{kpc}}                    % kpc
\def\Lsun{\ifmmode \un{L}_{\odot}     % solar luminosity
          \else $\un{L}_{\odot}$
          \fi}
\def\MHz{\un{MHz}}                    % MHz
\def\mJy{\un{mJy}}                    % mJy
\def\Mpc{\un{Mpc}}                    % Mpc
\def\Msun{\ifmmode \un{M}_{\odot}     % solar mass
          \else $\un{M}_{\odot}$
          \fi}
\def\muJy{\ifmmode \unitspace\mu\mbox{\rm Jy} % microJansky
          \else $\unitspace\mu$Jy
          \fi}
\def\mum{\ifmmode \unitspace\mu\mbox{\rm m} % micron
         \else $\unitspace\mu$m
         \fi}
\def\nm{\un{nm}}                      % nm
\def\pc{\un{pc}}                      % pc
\def\pcm{\per{cm}}                    %   -1
                                      % cm
\def\pcmcub{\pun{cm}{-3}}             %   -3
                                      % cm
\def\pcmsqu{\pun{cm}{-2}}             %   -2
                                      % cm
\def\pyr{\pun{yr}{-1}}                %   -1
                                      % yr
\def\ps{\pun{s}{-1}}                  %  -1
                                      % s
\def\sqarcsec{\ifmmode \unitspace\Box''    %       2
              \else $\unitspace\Box''$     % arcsec
              \fi} 

%
%-------------------------- quantities ---------------------------------------
%

\def\Bp{\relax                            % B
        \ifmmode B_{||}                   %  ||
        \else $B_{||}$
        \fi}
\def\Bt{\relax                            % B
        \ifmmode B\!_{\perp}              %  |
        \else $B\!_{\perp}$               %  -
        \fi}
\def\Dec{\relax                           % Dec
          \ifmmode \mbox{\rm Dec}
          \else Dec
         \fi}
\def\Eup{\relax                           % E
         \ifmmode E_{\rm u}               %  u
         \else $E_{\rm u}$
         \fi}
\def\Gcr{\relax                           % Gamma
         \ifmmode \Gamma\!_{\rm cr}       %      cr
         \else $\Gamma\!_{\rm cr}$
         \fi}
\def\ICII{\relax                          % I
          \ifmmode I_{[\CII]}             %  [C II]
          \else $I_{[\CII]}$
          \fi}
\def\LHtwo{\relax                                 % L
           \ifmmode L_{\mbox{\rm\scriptsize H}_2} %  H
           \else $L_{\mbox{\rm\scriptsize H}_2}$  %   2
           \fi}
\def\LFIR{\relax                           % L
          \ifmmode L_{\rm FIR}             %  FIR
          \else $L_{\rm FIR}$
          \fi}
\def\LIR{\relax                           % L
         \ifmmode L_{\rm IR}              %  IR
         \else $L_{\rm IR}$
         \fi}
\def\LLya{\relax                          % L
          \ifmmode L_{{\rm Ly}\,\alpha}   %  Ly alpha
          \else $L_{{\rm Ly}\,\alpha}$
          \fi}
\def\mAB{\relax                           % m
         \ifmmode m_{\rm AB}              %  AB
         \else $m_{\rm AB}$
         \fi}
\def\mHI{\relax                                      % m
         \ifmmode m_{\mbox{\scriptsize\rm H\,\sc I}} %  HI
         \else $m_{\mbox{\scriptsize\rm H\,\sc I}}$
         \fi}
\def\MHII{\relax                                       % M
          \ifmmode M_{\mbox{\scriptsize\rm H\,\sc II}} %  HII
          \else $M_{\mbox{\scriptsize\rm H\,\sc II}}$
          \fi}
\def\MHtwo{\relax                                 % M
           \ifmmode M_{\mbox{\rm\scriptsize H}_2} %  H
           \else $M_{\mbox{\rm\scriptsize H}_2}$  %   2
           \fi}
\def\MHtwodot{\relax                                       % .
              \ifmmode \dot{M}_{\mbox{\rm\scriptsize H}_2} % M
              \else $\dot{M}_{\mbox{\rm\scriptsize H}_2}$  %  H
              \fi}                                         %   2
\def\Mstardot{\relax                      % .
              \ifmmode \dot{M}_{\ast}     % M
              \else $\dot{M}_{\ast}$      %  *
              \fi}
\def\nH{\relax                                       % n
        \ifmmode n_{\mbox{\scriptsize\rm H}}  %  H
        \else $n_{\mbox{\scriptsize\rm H}}$
        \fi}
\def\nHI{\relax                                      % n
         \ifmmode n_{\mbox{\scriptsize\rm H\,\sc I}} %  HI
         \else $n_{\mbox{\scriptsize\rm H\,\sc I}}$
         \fi}
\def\nHt{\relax                                % n
         \ifmmode n_{{\mbox{\scriptsize H}}_2} %  H
         \else $n_{{\mbox{\scriptsize H}}_2}$  %   2
         \fi}
\def\RA{\relax                           % RA
         \ifmmode \mbox{\rm RA}
         \else RA
        \fi}
\def\rhostardot{\relax                         %  .
                \ifmmode \dot{\rho}_{\ast}     % rho
                \else $\dot{\rho}_{\ast}$      %    *
                \fi}
\def\rhoZdot{\relax                          %  .
             \ifmmode \dot{\rho}_{\rm Z}     % rho
             \else $\dot{\rho}_{\rm Z}$      %    Z
             \fi}
\def\Tb{\relax                           % T
        \ifmmode T_{\rm b}               %  b
        \else $T_{\rm b}$
        \fi}
\def\Tc{\relax                           % T
        \ifmmode T_{\rm c}               %  c
        \else $T_{\rm c}$
        \fi}
\def\Td{\relax                           % T
        \ifmmode T_{\rm d}               %  d
        \else $T_{\rm d}$
        \fi}
\def\Te{\relax                           % T
        \ifmmode T_{\rm e}               %  e
        \else $T_{\rm e}$
        \fi}
\def\Tg{\relax                           % T
        \ifmmode T_{\rm g}               %  g
        \else $T_{\rm g}$
        \fi}
\def\Tkin{\relax                         % T
          \ifmmode T_{\rm kin}           %  kin
          \else $T_{\rm kin}$
          \fi}
\def\Ts{\relax                           % T
        \ifmmode T_{\rm s}               %  s
        \else $T_{\rm s}$
        \fi}
\def\vhel{\relax                  %
          \ifmmode \qu{v}{hel}    % v
          \else $\qu{v}{hel}$     %  hel
          \fi}
\def\vLSR{\relax                  %
          \ifmmode \qu{v}{LSR}    % v
          \else $\qu{v}{LSR}$     %  LSR
          \fi}

%
%------------------ source designations -------------------------
%

\def\sou#1#2{\relax                       % source designations
             \ifmmode {\rm #1}\,{\rm #2}  % e.g. \sou{Arp}{220}
             \else #1$\,$#2
             \fi}

\def\APM#1{\sou{APM}{#1}}                % APM number

\def\Arp#1{\sou{Arp}{#1}}                % Arp number

\def\HD#1{\sou{HD}{#1}}                  % HD number

\def\HH#1{\sou{HH}{#1}}                  % HH number

\def\IC#1{\sou{IC}{#1}}                  % IC number

\def\IRAS#1{\sou{IRAS}{#1}}              % IRAS number

\def\Mrk#1{\sou{Mrk}{#1}}                % Mrk number

\def\NGC#1{\sou{NGC}{#1}}                % NGC number

\def\SMM#1{\sou{SMM}{#1}}                % SMM number

\def\UGC#1{\sou{UGC}{#1}}                % UGC number

%
%------------------- generic quantity symbols ------------------
%

\def\qu#1#2{\relax                          % quantity symbols
            \ifmmode #1_{\rm #2}            % e.g. \qu{L}{FIR}
            \else $#1_{\rm #2}$
            \fi}

\endinput

